GibbsDDRM: A Partially Collapsed Gibbs Sampler for Solving Blind Inverse Problems with Denoising Diffusion Restoration

Pre-trained diffusion models have been successfully used as priors in a variety of linear inverse problems, where the goal is to reconstruct a signal from noisy linear measurements. However, existing approaches require knowledge of the linear operator. In this paper, we propose GibbsDDRM, an extension of Denoising Diffusion Restoration Models (DDRM) to a blind setting in which the linear measurement operator is unknown. GibbsDDRM constructs a joint distribution of the data, measurements, and linear operator by using a pre-trained diffusion model for the data prior, and it solves the problem by posterior sampling with an efficient variant of a Gibbs sampler. The proposed method is problem-agnostic, meaning that a pre-trained diffusion model can be applied to various inverse problems without fine-tuning. In experiments, it achieved high performance on both blind image deblurring and vocal dereverberation tasks, despite the use of simple generic priors for the underlying linear operators.

==> theorems/prop_marginal_q_x_t.tex <==
The conditional distribution $q^{(t)}$ defined in Eqs.~\eqref{eq:gibbsDDRM_qT} and~\eqref{eq:gibbsDDRM_qt} satisfy the following:
\begin{align}
    q(\mathbf{x}_{t}|\mathbf{x}_{0}, \bm{\varphi}) = \mathcal{N}(\mathbf{x}_{0}, \sigma_{t}^{2}\bm{I}),
\end{align}
defined by marginalizing over $\mathbf{x}_{t'}$ (for all $t' > t$), $\mathbf{y}$, where $p(\mathbf{y}|\mathbf{x}_{0}, \bm{\varphi})$ is defined as in Eq.~\eqref{eq:mes_model} with $\mathbf{x}=\mathbf{x}_{0}$.

